GenoTEX: An LLM Agent Benchmark for Automated Gene Expression Data Analysis

Recent advancements in machine learning have significantly improved the identification of disease-associated genes from gene expression datasets. However, these processes often require extensive expertise and manual effort, limiting their scalability. Large Language Model (LLM)-based agents have shown promise in automating these tasks due to their increasing problem-solving abilities. To support the evaluation and development of such methods, we introduce GenoTEX, a benchmark dataset for the automated analysis of gene expression data. GenoTEX provides analysis code and results for solving a wide range of gene-trait association problems, encompassing dataset selection, preprocessing, and statistical analysis, in a pipeline that follows computational genomics standards. The benchmark includes expert-curated annotations from bioinformaticians to ensure accuracy and reliability. To provide baselines for these tasks, we present GenoAgent, a team of LLM-based agents that adopt a multi-step programming workflow with flexible self-correction, to collaboratively analyze gene expression datasets. Our experiments demonstrate the potential of LLM-based methods in analyzing genomic data, while error analysis highlights the challenges and areas for future improvement. We propose GenoTEX as a promising resource for benchmarking and enhancing automated methods for gene expression data analysis. The benchmark is available at https://github.com/Liu-Hy/GenoTEX.

==> secs/caseStudy.tex <==
\hwc{these were just place holders back then, we can get rid of it now.}
To offer a more direct understanding of 
the performances of our TAIS system, 
we detail a case study of one particular research question here. 
When our system is asked with 
``What genes are associated with Pancreatic Cancer when considering conditions related to Vitamin D Levels?''
Our system identified 20+ genes
with a disease (Pancreatic Cancer) prediction cross-validation accuracy 
of $80\%$. 

The top five genes identified are 
\textit{SLC11A1}, \textit{SOCS1}, \textit{CD207}, 
\textit{LILRB3}, and \textit{SPA17}.
Out of these five genes, four are implicated with 
Pancreatic Cancer when considering the interaction 
with Vitamin D Levels. 

\textit{SLC11A1} has been implicated in the host's response to pathogens and may also play a role in inflammatory diseases \cite{awomoyi2007human}. Given that inflammation is a known risk factor for pancreatic cancer, and vitamin D is involved in modulating inflammatory responses \cite{colotta2017modulation}, \textit{SLC11A1} could be a link between vitamin D levels and inflammation-related pancreatic cancer risk.

\textit{SOCS1} is a critical regulator of cytokine signaling pathways, including those involved in immune responses and inflammation \cite{ying2019socs1}. Vitamin D is known to modulate immune function \cite{baeke2010vitamin} and inflammation \cite{colotta2017modulation}, suggesting that SOCS1 could be part of the pathway through which vitamin D influences pancreatic cancer risk or progression.

\textit{CD207} is a C-type lectin receptor expressed on Langerhans cells, which are involved in immune responses in the skin but might also play roles in other types of immune responses. While the direct link between CD207, vitamin D, and pancreatic cancer is less clear, the potential connection might relate to the broader immune modulation by vitamin D and how it could affect cancer immunosurveillance.

\textit{LILRB3} is involved in the regulation of immune responses, including the inhibition of various cell signaling pathways. Vitamin D has been shown to influence the immune system \cite{baeke2010vitamin}, and alterations in LILRB3 function could potentially affect how the immune system responds to cancer cells in the context of varying vitamin D levels.

\textit{SPA17} is known for its expression in reproductive tissues and certain cancers. It may play a role in cancer cell mobility and immune evasion. Given vitamin D's effects on immune function \cite{baeke2010vitamin}, there could be a link between vitamin D levels and the immune response to pancreatic cancer cells expressing SPA17, impacting the disease's progression or response to therapy.

